Clinical Text Prediction with Numerically Grounded Conditional Language Models

Assisted text input techniques can save time and effort and improve text quality. In this paper, we investigate how grounded and conditional extensions to standard neural language models can bring improvements in the tasks of word prediction and completion. These extensions incorporate a structured knowledge base and numerical values from the text into the context used to predict the next word. Our automated evaluation on a clinical dataset shows extended models significantly outperform standard models. Our best system uses both conditioning and grounding, because of their orthogonal benefits. For word prediction with a list of 5 suggestions, it improves recall from 25.03% to 71.28% and for word completion it improves keystroke savings from 34.35% to 44.81%, where theoretical bound for this dataset is 58.78%. We also perform a qualitative investigation of how models with lower perplexity occasionally fare better at the tasks. We found that at test time numbers have more influence on the document level than on individual word probabilities.

==> comments.tex <==
=====R1=====

* IRB approval (or equivalent) - since this study is performed on authentic medical data, it is important to mention how access to the data was given. Is the dataset (or parts of it) publicly available, e.g. resulting vocabulary?
* KB - please describe this in more detail, how it was created/generated etc.

* Is the numerical issue specific to the clinical domain, and/or to this specific dataset? Could results be compared to other types of text, or at least to a (more) publicly available clinical corpus? Could you provide some additional examples of this particular characteristic of this dataset?

* A more general question: would these results be sufficient for "human acceptance", or do you think system performance (wrt e.g. F1) needs to be closer to the theoretical bound?

=====R2=====

L348: 'e.g.  a': You probably need a LaTeX soft stop here.

=====R3=====

How was the KB constructed?

I'm not familiar with research demonstrating that clinical text prediction software impacts patient care or makes clinicians more efficient.  Is there research that shows this is a good idea? Seems that this could be useful for target IE tasks, but is this something that clinicians would want to use?
The major limitation of this work is practical relevance.  Although the paper describes a new approach that shows notable improvements over a reference method, it is not clear the application is beneficial to clinical documentation processes or to patient care.
Even if the task were justified, the precision is too low to be used in practice. Also, there are a number of important operational/cultural considerations involved with the implementation of such a system in the healthcare setting that this paper ignores. A better justification for the research would improve the health/medical relevance of this paper.

- title is very general, but work seems very specific, and is restricted to a relatively small subset of all clinical notes (.
- no study limitations?  what about generalizability to new institutions?

-----------------------------------------------------------------------------------------------




============================================================================
                            REVIEWER #1
============================================================================


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------

                         Appropriateness: 5
                                 Clarity: 3
                             Originality: 3
                 Soundness / Correctness: 4
               Impact of Ideas / Results: 4
                   Meaningful Comparison: 4
                               Substance: 4
                           Replicability: 2
                          Recommendation: 4
                     Reviewer Confidence: 3
                     Presentation Format: Oral


---------------------------------------------------------------------------
Comments
---------------------------------------------------------------------------

The author(s) present a study on text prediction applied on clinical text, and
introduce a numerically grounded conditional language model. Results are
evaluated on a corpus of clinical text from the London Chest Hospital. The main
contribution of this work is the introduction of the conditional and
numerically grounded model for this task, and an in-depth analysis of the
behaviour of the model.

The manuscript is in general very well-written and the experimental and
methodological setup is sound. The study is very interesting and addresses an
important research problem in clinical NLP. As the author(s) mention in the
concluding section, alternative ways of representing/modeling/encoding
numerical information would be very interesting to study further.

There are a few issues that would benefit from being clarified or described in
some more detail:

* IRB approval (or equivalent) - since this study is performed on authentic
medical data, it is important to mention how access to the data was given. Is
the dataset (or parts of it) publicly available, e.g. resulting vocabulary?
* KB - please describe this in more detail, how it was created/generated etc.
* Is the numerical issue specific to the clinical domain, and/or to this
specific dataset? Could results be compared to other types of text, or at least
to a (more) publicly available clinical corpus? Could you provide some
additional examples of this particular characteristic of this dataset?
* A more general question: would these results be sufficient for "human
acceptance", or do you think system performance (wrt e.g. F1) needs to be
closer to the theoretical bound?

There are some minor errors in the manuscript, e.g.:
* 3.1: has a clear intention of typing a specific work and the --> word
* 3.2: We straightforwardly set --> remove "straightforwardly"?
* 5.3: Figure 3 --> Table 3
* Table 4: "non-dilatad" is misspelled - was this due to misspellings occuring
in the dataset?
* 5.4: We found that the changing the values does not have --> We found that
changing the values does not have
* 5.4: much more parameters have been used to model --> many more
* 5.4: changes in the the document probability --> changes in the document
probability
* 6: system performance in the two downstream tasks Our ablation --> missing
punctuation
* References: A et al. Tavast. 2012. --> this reference is inaccurate

============================================================================
                            REVIEWER #2
============================================================================


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------

                         Appropriateness: 5
                                 Clarity: 5
                             Originality: 3
                 Soundness / Correctness: 5
               Impact of Ideas / Results: 4
                   Meaningful Comparison: 5
                               Substance: 4
                           Replicability: 4
                          Recommendation: 4
                     Reviewer Confidence: 3
                     Presentation Format: Oral


---------------------------------------------------------------------------
Comments
---------------------------------------------------------------------------

General comments:

The authors describe a method for incorporating a structured knowledge base
into a word completion and prediction model. Particular emphasis is given to
the treatment of numerical values in the text. Their extended model is shown to
outperform standard models.

The paper is very well written and easy to follow. It presented useful ideas
for integrating context, which may be applicable for other domains than word
completion and prediction. It would have been nice to have some additional
description of the baseline neural language model (referred to in L284) since
the publication title was anonymised away - but this is not a problem for the
published paper.

Specific comments:

L241: 'work' => 'word'.

L267: I would have liked an explanation of the term 'one-hot'.

L348: 'e.g.  a': You probably need a LaTeX soft stop here.

L747: Missing period after 'tasks'.

L748: 'qualitatiuve' => 'qualitative'.

============================================================================
                            REVIEWER #3
============================================================================


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------

                         Appropriateness: 5
                                 Clarity: 4
                             Originality: 4
                 Soundness / Correctness: 4
               Impact of Ideas / Results: 3
                   Meaningful Comparison: 5
                               Substance: 4
                           Replicability: 3
                          Recommendation: 4
                     Reviewer Confidence: 4
                     Presentation Format: Oral


---------------------------------------------------------------------------
Questions for Authors
---------------------------------------------------------------------------

How was the KB constructed?

I'm not familiar with research demonstrating that clinical text prediction software impacts patient care or makes clinicians more efficient.  Is there research that shows this is a good idea?  Seems that this could be useful for target IE tasks, but is this something that clinicians would want to use?

---------------------------------------------------------------------------
Comments
---------------------------------------------------------------------------

This work applies state-of-the-art methods to the task of clinical text
prediction.  The work is interesting methodologically and clearly presented.
Also, the study appears to be solid and the analysis is thorough.

The major limitation of this work is practical relevance.  Although the paper
describes a new approach that shows notable improvements over a reference
method, it is not clear the application is beneficial to clinical documentation
processes or to patient care.  Even if the task were justified, the precision
is too low to be used in practice.  Also, there are a number of important
operational/cultural considerations involved with the implementation of such a
system in the healthcare setting that this paper ignores.  A better
justification for the research would improve the health/medical relevance of
this paper.

Other points:

- title is very general, but work seems very specific, and is
restricted to a relatively small subset of all clinical notes (.
- some typos and structural issues.  For example, the abstract states that the
best system used grounding and conditioning b/c of the "orthogonal benedicts".
- no study limitations?  what about generalizability to new institutions?

==> figures/conditional_example.tex <==
\begin{figure}%[htp]
\centering
\includegraphics[width=0.5\textwidth]{bar_chart}
\caption{Qualitative example. Template and probabilities of $<$WORD$>$=\{`non', `mildly', `severely'\} for varying numbers.}
%\caption{Qualitative example. \underline{top}: text; \underline{bottom:} normalised probabilities for $<$WORD$>$=\{'non', 'mildly', 'severely'\} for numbers consistent with ejection fraction EF=65\% (left), EF=2.5\% (middle) and EF=0.5\% (right).}
\label{fig:conditional_example}
\end{figure}

==> tables/kb_statistics.tex <==
\begin{table}%[h!]
\centering
 \begin{tabular}{r r r r r r} 
 \hline
 & & & \bf train & \bf dev & \bf test \\ [0.5ex]
 \hline
 %--------------------------------------
 \multicolumn{3}{r}{\#documents} & 11,158 & 1,625 & 3,220 \\
 \hline
 
 %--------------------------------------
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\#tokens/}}}
 &
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{doc}}}
 & all & 204.9 & 204.4 & 202.2\\
 %& & words & 196.1 & 195.6 & 193.5\\
 & & words & 95.7\% & 95.7\% & 95.7\%\\
 %& & numeric & 8.8 & 8.8 & 8.7\\
 & & numeric & 4.3\% & 4.3\% & 4.3\%\\
 \hline
 %--------------------------------------
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{OOV}}}
 &
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{rate}}}
 & all & 5.0\% & 5.1\% & 5.2\%\\
 & & words & 3.4\% & 3.5\% & 3.5\%\\
 & & numeric & 40.4\% & 40.8\% & 41.8\%\\
 \hline
 %--------------------------------------

 \end{tabular}
 \caption{Statistics for clinical dataset. Counts for non-numeric (\textit{words}) and \textit{numeric} tokens reported as percentage of counts for \textit{all} tokens. Out-of-vocabulary (OOV) rates are for vocabulary of $1000$ most frequent words in the train data.
 }
 \label{tab:kb_statistics}
\end{table}
